Embodied Language Grounding with 3D Visual Feature Representations

We propose associating language utterances to 3D visual abstractions of the scene they describe. The 3D visual abstractions are encoded as 3-dimensional visual feature maps. We infer these 3D visual scene feature maps from RGB images of the scene via view prediction: when the generated 3D scene feature map is neurally projected from a camera viewpoint, it should match the corresponding RGB image. We present generative models that condition on the dependency tree of an utterance and generate a corresponding visual 3D feature map as well as reason about its plausibility, and detector models that condition on both the dependency tree of an utterance and a related image and localize the object referents in the 3D feature map inferred from the image. Our model outperforms models of language and vision that associate language with 2D CNN activations or 2D images by a large margin in a variety of tasks, such as, classifying plausibility of utterances, detecting referential expressions, and supplying rewards for trajectory optimization of object placement policies from language instructions. We perform numerous ablations and show the improved performance of our detectors is due to its better generalization across camera viewpoints and lack of object interferences in the inferred 3D feature space, and the improved performance of our generators is due to their ability to spatially reason about objects and their configurations in 3D when mapping from language to scenes.

==> 1_abstract_old.tex <==

\begin{abstract}


%This hypothesis is currently better known as 
%The hypothesis of simulation semantics suggests that people think and reason about language utterances visually. It 
%formally  states that  processing words and sentences leads to perceptual and motor simulations of  %Simul 
%explicitly and implicitly mentioned aspects of linguistic content.  
We  propose 
associating language utterances to 3D visual abstractions of the scene they describe. 
The 3D visual abstractions are encoded as a 3-dimensional visual feature maps. 
We infer such 3D visual scene feature maps from  RGB images of the scene via view prediction: the generated 3D scene feature map when neurally projected from a camera viewpoint it should  match the corresponding RGB image. 

We present language to mental imagination generative models that  
The models we propose have two functionalities: i) conditioned on the dependency tree of an utterance, they generate the related visual 3D feature map and reason about its plausibility (without access to any visual input), and ii) conditioned on the dependency tree of a referential expression and a related image they localize object referents in the   3D feature map inferred from the  image.  
We empirically show   our model outperforms by a large margin models of language and vision that associate language with 2D CNN activations or 2D images in a variety of tasks, such as, 
 classifying plausibility of utterances by spatially reasoning over possible and impossible object configurations, 3D object referential detection, inferring desired scene transformations given  language instructions, and   providing rewards for trajectory optimization of corresponding policies.  We attribute the improved performance of our model to its  improved  generalization across   camera viewpoints and reasoning of possible object arrangements, benefits of its 3D visual grounding space, in place of view-dependent images and CNN  image features. 



\end{abstract}



\begin{abstract}



%\begin{comment}
%When we read or hear a natural language utterance, e.g., 
%Consider the utterance \textit{``He used the newspaper to protect his face from the wind''.} Humans can  answer numerous questions about the situation  described, as well as reason through counterfactuals and alternatives, such as: \textit{`` How many free hands does the man have? How many pages the newspaper should have for  adequate wind protection? Does the newspaper protect also the man's legs? If yes, the man should be cuddled behind it"}, and so on. Even much simpler sentences, such as, 

Consider the utterance \textit{``the tomato is to the left of the pot"}. Humans can  answer numerous questions about the situation  described, as well as reason through counterfactuals and alternatives, such as, \textit{``is the pot larger than the tomato?", ``can we move to a viewpoint from which the tomato is completely hidden behind the pot?", ``can we have an object that is both to the left of the tomato and to the right of the pot?", ``would the tomato fit inside the pot?"}
%Consider the utterance \textit{``the tomato is to the left of the pot"}. Humans can  answer numerous questions about the situation  described, as well as reason through counterfactuals and alternatives, such as, \textit{``is the pot larger than the tomato?", ``can we move to a viewpoint from which the tomato is completely hidden behind the pot?", ``can we have an object that is both to the left of the tomato and to the right of the pot?", ``would the tomato fit inside the pot?"}
, and so on.  Such  reasoning capability remains  elusive from current  computational models of language understanding. %, despite tremendous progress  
%It is further unclear what supervision is necessary for such reasoning ability to emerge.
%how to teach machines such versatile reasoning capability through a question-answering pairs type of supervision over images and their corresponding CNN 2D feature representations. 
%: there is simply too much information about object sizes, arrangements, occlusion relationships and so on, to capture through question answers. It has been argued that humans link language to mental pictures of the  experience described. Such mental visual simulations trigger such reasoning. 
%Indeed, a picture is  1000 words, if not more. 
%To enable basic  reasoning over  language of object 
To link language processing with spatial reasoning, we propose associating natural language utterances to a mental workspace of their meaning, encoded as  3-dimensional visual feature representations of the world scenes they describe. %, and show how such associations permits spatial reasoning over a language domain of object spatial arrangements. %, akin to 3D abstract visual imaginations.      
%In this work, we show how visual embodiment---the ability to see a scene from multiple viewpoints---helps inject spatial common sense  in   understanding language of object spatial arrangements.  
%We propose 
%mapping  natural language utterances to a mental workspace of their meaning, encoded as a 3-dimensional visual feature representations.     
%We propose grounding  natural language utterances to  compositional  3-dimensional visual abstractions of their meaning. 
We  learn such  3-dimensional visual representations---we call them visual imaginations--- by  predicting images a mobile agent sees while moving around in the 3D world. The input image streams the agent collects are {\it  unprojected} into egomotion-stable  3D scene feature maps of the scene, and projected from novel viewpoints to match the observed RGB image views in an end-to-end differentiable manner.% when projected from the corresponding camera viewpoints. %while disentangling scenetht learn to map 2D image streams to 3D features representations of the scene, while disentangling them from camera motion by a mobile agent trained to predict  image views while moving in the world scene. 
%The 3D feature maps retain perceptual  information regarding appearance, size, occupancy, 3D shape, spatial arrangements and geometry of the objects in the scene. %After training, our agent can map a 2D RGB stream or single RGB image  to a  3D feature map of the scene,  completing by imagination occluded information. 
%Given a set of scenes annotated with natural language descriptions, we train  generative networks to map the textual descriptions  to the corresponding 3-dimensional visual feature maps, in a modular, object-factorized way. %Given a set of scenes annotated with object referential expressions, we train discriminative networks to map the referrentials  to the referred 3D object boxes in the inferred 3D feature maps. 
% and are supervised by an embodied agents trained to predict RGB results of its egomotion.
%We present  stochastic generative networks that, condition on a natural language utterance,  generate   3-dimensional feature maps of the referred  scene,  one object  at a time.
%,  place them into a 4D feature canvas, which, when projected from  various viewpoints   matches the corresponding RGB views. 
%When the composed 3D feature maps are projected from various viewpoints they need to be decodable to corresponding RGB images. 
%The  3-dimensional object-centric feature representations of noun phrases operate as visual detectors and localize the referents in the agent's environment, when present. 
%In this way, our model combines perception and imagination and can generate scenes conditioning on both a language utterance and the visual environment of the agent, necessary for instruction following, e.g., ``move the cylinder to the left of the  blue sphere". 
We then train modular neural models to generate  such 3D feature representations given language utterances, to localize the objects an utterance mentions in the 3D feature representation inferred from an image, and to predict the desired 3D object  locations given a manipulation instruction. %, and use the latter for trajectory optimization and policy . %show we can of obtaining the corresponding policy. %given a sentence describing the scene.
%referential expressions on image. 
We empirically show the proposed models 
%grounding can reason about plausibility and implausibility of utterances,   localize object referents in 3D across varying camera viewpoints,   and execute manipulation linguistic instructions by inferring desired object locations in 3D used for trajectory optimization. They 
outperform by a large margin existing 2D  models in spatial reasoning, referential object detection and instruction following, and generalize better across camera viewpoints and  object arrangements.


%all the above tasks.





%Though current visual question answering systems have shown a continuing performance over the past years, existing computational models of language and vision often very basic facts about the world, so basic that they are not annotated in the question-answering datasets, for example, the fact that objects do not 3D intersect, that objects persist and do not spontaneously disappear, that an object appears larger when closer to the camera but retains a world size, and so on.
%does a man sitting in a desk have legs, how long. 
%For example, they 




%\begin{comment}
%When we read or hear a natural language utterance, e.g., 
%Consider the utterance \textit{``He used the newspaper to protect his face from the wind''.} Humans can  answer numerous questions about the situation  described, as well as reason through counterfactuals and alternatives, such as: \textit{`` How many free hands does the man have? How many pages the newspaper should have for  adequate wind protection? Does the newspaper protect also the man's legs? If yes, the man should be cuddled behind it"}, and so on. Even much simpler sentences, such as, 
%``can we move to a viewpoint from which the tomato is completely hidden behind the pot?",``would the tomato fit inside the pot?"
Consider the utterance \textit{``the tomato is to the left of the pot"}. Humans can  answer numerous questions about the situation  described, as well as reason through counterfactuals and alternatives, such as, \textit{``is the pot larger than the tomato?", ``can we move to a viewpoint from which the tomato is completely hidden behind the pot?", ``can we have an object that is both to the left of the tomato and to the right of the pot?", ``would the tomato fit inside the pot?"}
%Consider the utterance \textit{``the tomato is to the left of the pot"}. Humans can  answer numerous questions about the situation  described, as well as reason through counterfactuals and alternatives, such as, \textit{``is the pot larger or smaller than the tomato?",  ``can we have an object that is both to the left of the tomato and to the right of the pot?," ``can we see the tomato if we view from the side or from the top?''}, and so on.  Such  reasoning capability remains  elusive from current computational models of language understanding. %, despite tremendous progress  
%It is further unclear what supervision is necessary for such reasoning ability to emerge.
%how to teach machines such versatile reasoning capability through a question-answering pairs type of supervision over images and their corresponding CNN 2D feature representations. 
%: there is simply too much information about object sizes, arrangements, occlusion relationships and so on, to capture through question answers. It has been argued that humans link language to mental pictures of the  experience described. Such mental visual simulations trigger such reasoning. 
%Indeed, a picture is  1000 words, if not more. 
%To enable basic  reasoning over  language of object 
To link language processing with spatial reasoning, we propose associating natural language utterances to a mental workspace of their meaning, encoded as  3-dimensional visual feature representations of the world scenes they describe. %, and show how such associations permits spatial reasoning over a language domain of object spatial arrangements. %, akin to 3D abstract visual imaginations.      
%In this work, we show how visual embodiment---the ability to see a scene from multiple viewpoints---helps inject spatial common sense  in   understanding language of object spatial arrangements.  
%We propose 
%mapping  natural language utterances to a mental workspace of their meaning, encoded as a 3-dimensional visual feature representations.     
%We propose grounding  natural language utterances to  compositional  3-dimensional visual abstractions of their meaning. 
We learn such  3-dimensional visual representations---we call them visual imaginations--- by  predicting images a mobile agent sees while moving around in the 3D world. The input image streams the agent collects are {\it  unprojected} into egomotion-stable  3D scene feature maps of the scene, and projected from novel viewpoints to match the observed RGB image views in an end-to-end differentiable manner.
%The input image streams the agent collects are {\it  unprojected} into egomotion-stable  3D scene feature maps of the scene, and projected from novel viewpoints to match the observed RGB image views in an end-to-end differentiable manner.
% when projected from the corresponding camera viewpoints. %while disentangling scenetht learn to map 2D image streams to 3D features representations of the scene, while disentangling them from camera motion by a mobile agent trained to predict  image views while moving in the world scene. 
%The 3D feature maps retain perceptual  information regarding appearance, size, occupancy, 3D shape, spatial arrangements and geometry of the objects in the scene. %After training, our agent can map a 2D RGB stream or single RGB image  to a  3D feature map of the scene,  completing by imagination occluded information. 
%Given a set of scenes annotated with natural language descriptions, we train  generative networks to map the textual descriptions  to the corresponding 3-dimensional visual feature maps, in a modular, object-factorized way. %Given a set of scenes annotated with object referential expressions, we train discriminative networks to map the referrentials  to the referred 3D object boxes in the inferred 3D feature maps. 
% and are supervised by an embodied agents trained to predict RGB results of its egomotion.
%We present  stochastic generative networks that, condition on a natural language utterance,  generate   3-dimensional feature maps of the referred  scene,  one object  at a time.
%,  place them into a 4D feature canvas, which, when projected from  various viewpoints   matches the corresponding RGB views. 
%When the composed 3D feature maps are projected from various viewpoints they need to be decodable to corresponding RGB images. 
%The  3-dimensional object-centric feature representations of noun phrases operate as visual detectors and localize the referents in the agent's environment, when present. 
%In this way, our model combines perception and imagination and can generate scenes conditioning on both a language utterance and the visual environment of the agent, necessary for instruction following, e.g., ``move the cylinder to the left of the  blue sphere". 
We then train modular neural models to generate  such 3D feature representations given language utterances, to localize the objects an utterance mentions in the 3D feature representation inferred from an image, and to predict the desired 3D object  locations given a manipulation instruction. %, and use the latter for trajectory optimization and policy . %show we can of obtaining the corresponding policy. %given a sentence describing the scene.
%referential expressions on image. 
We empirically show the proposed models 
%grounding can reason about plausibility and implausibility of utterances,   localize object referents in 3D across varying camera viewpoints,   and execute manipulation linguistic instructions by inferring desired object locations in 3D used for trajectory optimization. They 
outperform by a large margin existing 2D  models in spatial reasoning, referential object detection and instruction following, and generalize better across camera viewpoints and  object arrangements.


%all the above tasks.


%\end{comment}
\end{abstract}

\begin{comment}

\todo{
%Upon hearing the sentence ``putting the elephant in the refrigerator,'' most people start imagining a scene where they try to squeeze a gigantic elephant to a poor refrigerator, and soon realize the impossibility of doing this.


%there is simply too much information that is conveyed in the picture for our models to learn in a supervised way
%This type of knowledge is often called {\it common sense} since humans can obtain it without being taught and most people agree with the true/false of the statement. While humans develop common sense effortlessly, current machine learning
%algorithms struggle to do so and some of them even require carefully designed datasets which contains question-answer pairs obtained from real humans. This paper makes a step towards injecting spatial common sense into natural language understanding without the needs to learn from human annotated question-answer pairs.
%}




\todo{
We propose
mapping natural language to 3-dimensional visual feature abstractions of its meaning.    
These 3-dimensional visual abstractions 
are learned in an unsupervised way by Geometry-Aware Recurrent Networks (GRNNs) trained to predict images that an embodied agent sees while moving in a world scene \cite{commonsense}. The 3D feature maps retain perceptual  information regarding appearance, size, occupancy, 3D shape, spatial arrangements and geometry of the objects in the scene. 
To map languages to these 3D feature abstractions, we prepare a set of scenes annotated with natural language descriptions and train generative networks to map the textual descriptions  to the corresponding 3-dimensional visual feature maps, in a modular, object-factorized way. To find the object mentioned in a sentence, we train discriminative networks to map the referrentials to the referred 3D object boxes in the 3D feature maps. 
We show the proposed model can infer  plausibility and implausibility of utterances,  can localize object referents robust to camera viewpoint, can generalize both generation and detection to longer parse trees than training time,  can  predict target goal object locations in 3D for training policies to follow object placement instructions, and outperforms by a margin 2D baselines in all above tasks.
}

\end{comment}
